Enhanced Robot Planning and Perception through Environment Prediction

Mobile robots rely on maps to navigate through an environment. In the absence of any map, the robots must build the map online from partial observations as they move in the environment. Traditional methods build a map using only direct observations. In contrast, humans identify patterns in the observed environment and make informed guesses about what to expect ahead. Modeling these patterns explicitly is difficult due to the complexity of the environments. However, these complex models can be approximated well using learning-based methods in conjunction with large training data. By extracting patterns, robots can use direct observations and predictions of what lies ahead to better navigate an unknown environment. In this dissertation, we present several learning-based methods to equip mobile robots with prediction capabilities for efficient and safer operation. In the first part of the dissertation, we learn to predict using geometrical and structural patterns in the environment. Partially observed maps provide invaluable cues for accurately predicting the unobserved areas. We first demonstrate the capability of general learning-based approaches to model these patterns for a variety of overhead map modalities. Then we employ task-specific learning for faster navigation in indoor environments by predicting 2D occupancy in the nearby regions. This idea is further extended to 3D point cloud representation for object reconstruction. Predicting the shape of the full object from only partial views, our approach paves the way for efficient next-best-view planning. In the second part of the dissertation, we learn to predict using spatiotemporal patterns in the environment. We focus on dynamic tasks such as target tracking and coverage where we seek decentralized coordination between robots. We first show how graph neural networks can be used for more scalable and faster inference.

==> Abbreviations.tex <==
%List of Abbreviations

\renewcommand{\baselinestretch}{1}
\small\normalsize
\hbox{\ }

\vspace{.5in}


\begin{center}
\large{List of Abbreviations}
\end{center} 

\vspace{3pt}

\begin{tabular}{ll}
$\alpha$ & alpha \\
$\beta$  & beta \\
&  \\ 
IREAP & Institute for Research in Electronics and Applied Physics \\
NSA & National Security Agency
\end{tabular}


==> Preface.tex <==
%Preface
\pagestyle{plain}\pagenumbering{roman} \setcounter{page}{2}
\renewcommand{\baselinestretch}{2}
\small\normalsize
\hbox{\ }

\vspace{.5in}

\begin{center}
\large{Preface}
\end{center}


If needed.

% figs/Agent_House10_Itr1.png
% figs/Agent_House13_Itr1.png
% figs/C17Overview.png
% figs/CDL2-Uni_Obs_2_robots.png
% figs/CDL2-Uni_Obs_4_robots.png
% figs/CDL2-Uni_Obs_6_robots.png
% figs/CDL2_comparison_2_rob.pdf
% figs/CDL2_comparison_4_rob.pdf
% figs/CDL2_comparison_6_rob.pdf
% figs/FM_overview.PNG
% figs/FM_overview_multimodal.jpeg
% figs/FM_overview_multimodal.png
% figs/Flowchart_new.png
% figs/GAN_FullView_Pred.png
% figs/InitialObservedC17.png
% figs/InitialPredictedC17.png
% figs/Inspection_IROS23.png
% figs/MAP-NBV-Information.png
% figs/MA_Distance.png
% figs/MA_PointsObserved.png
% figs/MultiAgentExpl.pdf
% figs/a2t_models.pdf
% figs/ablation_on_steps.pdf
% figs/acc_histogram_gan.png
% figs/airsim_mapnbv_2_robots.png
% figs/all_method_comparison.pdf
% figs/all_method_comparison_horz.pdf
% figs/all_method_comparison_horz_updated.pdf
% figs/all_method_comparison_horz_updated_v2.pdf
% figs/apend_seg_indoor.png
% figs/arc_motions.dia
% figs/arc_motions.png
% figs/c2_pic.png
% figs/c3_pic.png
% figs/c4_pic.png
% figs/captured_image_0.jpg
% figs/cars1_rgb.png
% figs/cars1_seg.png
% figs/cars2_all.png
% figs/cars2_seg.png
% figs/cars3_all.png
% figs/cars4_all.png
% figs/cars5_all.png
% figs/classification_comparison.pdf
% figs/combined_pred_overview.png
% figs/decile_plot.jpg
% figs/decile_plot.pdf
% figs/decile_plot_rot.pdf
% figs/decile_plot_transl.pdf
% figs/example_flow.jpg
% figs/example_flow_v2.jpg
% figs/fig_1.png
% figs/fig_2.png
% figs/fig_3.png
% figs/fig_intro_new.pdf
% figs/fig_nav5.png
% figs/fig_ros_new.pdf
% figs/fig_wp_polar.png
% figs/fig_wpc.pdf
% figs/fliptd_overview.jpeg
% figs/fliptd_overview.png
% figs/fliptd_tasks.PNG
% figs/fliptd_tasks.jpeg
% figs/fp227_marked.png
% figs/fp227_mod.png
% figs/fp227_modified.png
% figs/fp227_orig.png
% figs/fp227_original.png
% figs/fullview_com.pdf
% figs/fullview_two_comp.pdf
% figs/ga_image.png
% figs/greset_dist.jpg
% figs/habitat_models.pdf
% figs/image_0_grid_100.jpg
% figs/image_0_grid_6.jpg
% figs/image_10_grid_100.jpg
% figs/image_15_grid_100.jpg
% figs/image_15_grid_6.jpg
% figs/image_23_.png
% figs/image_23_grid_10.jpg
% figs/image_23_grid_100.jpg
% figs/image_23_grid_150.jpg
% figs/image_23_grid_50.jpg
% figs/indoors_3fovs_size.PNG
% figs/inpainting.png
% figs/inpainting_risk_aware.jpeg
% figs/map_nbv_overview_v3.jpeg
% figs/map_nbv_oveview_v2.png
% figs/map_nbv_oveview_v3.png
% figs/mapnbv.png
% figs/models.png
% figs/mountain1_rgb.png
% figs/mountain1_seg.png
% figs/mountain2_seg.png
% figs/mountain3_all.png
% figs/multi_agent_explr_overview.png
% figs/obs_ex_camera.png
% figs/occmap_overview_v2.png
% figs/occmap_overview_v3.png
% figs/occmap_real.png
% figs/occmap_real_cropped.png
% figs/oracle_commlen_1_all_wordcloud.png
% figs/oracle_commlen_3_all_wordcloud.png
% figs/oracle_commlen_5_all_wordcloud.png
% figs/our_nbv_path.png
% figs/over_a.png
% figs/over_a_alt.png
% figs/over_a_alt2.png
% figs/over_b.png
% figs/over_b_alt.png
% figs/overb_alt.png
% figs/overview.png
% figs/overview_v2.png
% figs/proxmap_turtlebot.jpg
% figs/realworld_occmap.png
% figs/regression_comparison.pdf
% figs/result_plots.png
% figs/robot_view_alt.PNG
% figs/semanticSystemOverview.jpeg
% figs/semantic_gc_overview.png
% figs/small_time_comparison_v3.pdf
% figs/stirrer_yw.png
% figs/trajectory_airport.png
% figs/turtlebot2.png
% figs/uncertainity.png
% figs/zed_poses.png

